What Was Your Prompt? A Remote Keylogging Attack on AI Assistants

AI assistants are becoming an integral part of society, used for asking advice or help in personal and confidential issues. In this paper, we unveil a novel side-channel that can be used to read encrypted responses from AI Assistants over the web: the token-length side-channel. We found that many vendors, including OpenAI and Microsoft, have this side-channel. However, inferring the content of a response from a token-length sequence alone proves challenging. This is because tokens are akin to words, and responses can be several sentences long leading to millions of grammatically correct sentences. In this paper, we show how this can be overcome by (1) utilizing the power of a large language model (LLM) to translate these sequences, (2) providing the LLM with inter-sentence context to narrow the search space and (3) performing a known-plaintext attack by fine-tuning the model on the target model's writing style. Using these methods, we were able to accurately reconstruct 29\% of an AI assistant's responses and successfully infer the topic from 55\% of them. To demonstrate the threat, we performed the attack on OpenAI's ChatGPT-4 and Microsoft's Copilot on both browser and API traffic.

==> vendors.tex <==

\begin{table*}[]
\resizebox{\textwidth}{!}{
%def\arraystretch{.7}
\begin{tabular}{@{}llllllll@{}}
\toprule
Vendor          & Service                             & Models                             & Has   side channel & Is   vulnerable & Protocol          & Extraction   Method              & Buffering         \\ \midrule
OpenAI          & ChatGPT                             & GPT4,   GPT3.5                     & $\bullet$          & $\bullet$       & QUIC+TLS+UDP      & current   payload - last payload & frequent   / rare \\
                & GPTs   - Marketplace                & GPT4                               & $\bullet$          & $\bullet$       & QUIC+TLS+UDP      & current   payload - last payload & rare              \\
                & API                                 & GPT4                               & $\bullet$          & $\bullet$       & TLS+TCP           & payload                          & paired            \\
Microsoft       & Bing   Chat Copilot                 & GPT4                               & $\bullet$          & $\bullet$       & WebSocket+TLS+TCP & current   payload - last payload & rare              \\
Writesonic      & Chatsonic                           & GPT4                               & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & rare              \\
Anthropic       & Claude   AI                         & Claude-v2                          & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & rare              \\
Notion          & Notion   AI Copilot                 & ?                                  & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & paired            \\
ClickUp         & ClickUp   AI Brain                  & ?                                  & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & paired            \\
TextCortex      & TextCortex   AI Copilot             & ?                                  & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & paired            \\
CKSoruce        & CKEditor                            & ?                                  & $\bullet$          & $\bullet$       & HTTP2+TLS+TCP     & payload                          & paired            \\
Quora           & Poe                                 & GPT4,   GPT3.5, Claude-v2 and more & $\bullet$          & $\circ$       & WebSocket+TLS+TCP & current   payload - last payload & none              \\
Perplexity   AI & Perplexity   AI                     & GPT4,   GPT3.5, Claude-v2          & $\bullet$          & $\circ$       & WebSocket+TLS+TCP & current   payload - last payload & none              \\
CopyAI          & CopyAI & ?                                  & $\bullet$          & $\circ$       & WebSocket+TLS+TCP & current   payload - last payload & none              \\
Google          & Bard                                & Palm2                              & $-$                & $-$             & HTTP2+TLS+TCP     & ?                                & ?                 \\
Github          & Copilot                             & GPT-4   Turbo                      & $-$                & $-$             & TLS+TCP           & ?                                & ?                 \\ \bottomrule
\end{tabular}
}
\end{table*}
